Effect or Treatment Heterogeneity? Policy Evaluation with Aggregated and Disaggregated Treatments

Binary treatments are often ex-post aggregates of multiple treatments or can be disaggregated into multiple treatment versions. Thus, effects can be heterogeneous due to either effect or treatment heterogeneity. We propose a decomposition method that uncovers masked heterogeneity, avoids spurious discoveries, and evaluates treatment assignment quality. The estimation and inference procedure based on double/debiased machine learning allows for high-dimensional confounding, many treatments and extreme propensity scores. Our applications suggest that heterogeneous effects of smoking on birthweight are partially due to different smoking intensities and that gender gaps in Job Corps effectiveness are largely explained by differential selection into vocational training.

==> Tables/Results_gender.tex <==
\begin{table}[t]
\centering
 \caption{Heterogeneous Effects by Gender} 
  \label{tab:ols-gender} 
\begin{threeparttable}
\begin{tabular}{cccccc}
 \toprule
\multicolumn{2}{c}{$nATE$} & \multicolumn{2}{c}{$rATE$} & \multicolumn{2}{c}{$\Delta$} \\
Constant & Female & Constant & Female & Constant & Female \\ 
  \midrule
17.51 & -7.64 & 17.19 & -6.89 & 0.32 & -0.75 \\ 
(5.41) & (7.55) & (5.63) & (8.06) & (1.68) & (2.69) \\ 
\bottomrule
\end{tabular}
\begin{tablenotes} \item \textit{Note:} Table shows the results of OLS regressions with the $nATE$, $rATE$ and $\Delta$ pseudo-outcomes and a female indicator, respectively. Standard errors that adjust for the estimated version shares in $rATE$ and $\Delta$ are provided in parentheses. \end{tablenotes}  
\end{threeparttable}
\end{table}

==> figures/MC1PAR_tab_n1000.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Thu Feb 11 00:08:20 2021
\begin{subtable}[h]{0.45\textwidth}
\centering
\caption{n = 1000} 
\begin{tabular}{llrrr}
  \hline
 &  & $rATE$ & $nATE$ & $\Delta$ \\ 
  \hline
k = 10 & $\alpha$ & 0.9460 & 0.9456 & 0.9524 \\ 
   & $\beta$ & 0.9444 & 0.9488 & 0.9470 \\ 
  k = 100 & $\alpha$ & 0.9468 & 0.9488 & 0.9518 \\ 
   & $\beta$ & 0.8974 & 0.9434 & 0.9474 \\ 
   \hline
\end{tabular}
\end{subtable}


==> figures/MC1PAR_tab_n5000.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Thu Feb 11 00:08:20 2021
\begin{subtable}[h]{0.45\textwidth}
\centering
\caption{n = 5000} 
\begin{tabular}{llrrr}
  \hline
 &  & $rATE$ & $nATE$ & $\Delta$ \\ 
  \hline
k = 10 & $\alpha$ & 0.9486 & 0.9480 & 0.9482 \\ 
   & $\beta$ & 0.9448 & 0.9528 & 0.9570 \\ 
  k = 100 & $\alpha$ & 0.9506 & 0.9508 & 0.9508 \\ 
   & $\beta$ & 0.9380 & 0.9464 & 0.9458 \\ 
   \hline
\end{tabular}
\end{subtable}


==> figures/MC1_tab_n1000.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Wed Feb 10 22:25:18 2021
\begin{subtable}[h]{0.45\textwidth}
\centering
\caption{n = 1000} 
\begin{tabular}{llrrr}
  \hline
 &  & $rATE$ & $nATE$ & $\Delta$ \\ 
  \hline
k = 10 & $\alpha$ & 0.9472 & 0.9494 & 0.8964 \\ 
   & $\beta$ & 0.9456 & 0.9452 & 0.9430 \\ 
  k = 100 & $\alpha$ & 0.9438 & 0.9420 & 0.8538 \\ 
   & $\beta$ & 0.9486 & 0.9476 & 0.9542 \\ 
   \hline
\end{tabular}
\end{subtable}


==> figures/MC1_tab_n5000.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Wed Feb 10 22:25:18 2021
\begin{subtable}[h]{0.45\textwidth}
\centering
\caption{n = 5000} 
\begin{tabular}{llrrr}
  \hline
 &  & $rATE$ & $nATE$ & $\Delta$ \\ 
  \hline
k = 10 & $\alpha$ & 0.9516 & 0.9500 & 0.9326 \\ 
   & $\beta$ & 0.9498 & 0.9506 & 0.9478 \\ 
  k = 100 & $\alpha$ & 0.9512 & 0.9508 & 0.9204 \\ 
   & $\beta$ & 0.9534 & 0.9520 & 0.9534 \\ 
   \hline
\end{tabular}
\end{subtable}

